DroneNet: Crowd Density Estimation using Self-ONNs for Drones

Video surveillance using drones is both convenient and efficient due to the ease of deployment and unobstructed movement of drones in many scenarios. An interesting application of drone-based video surveillance is to estimate crowd densities (both pedestrians and vehicles) in public places. Deep learning using convolution neural networks (CNNs) is employed for automatic crowd counting and density estimation using images and videos. However, the performance and accuracy of such models typically depend upon the model architecture i.e., deeper CNN models improve accuracy at the cost of increased inference time. In this paper, we propose a novel crowd density estimation model for drones (DroneNet) using Self-organized Operational Neural Networks (Self-ONN). Self-ONN provides efficient learning capabilities with lower computational complexity as compared to CNN-based models. We tested our algorithm on two drone-view public datasets. Our evaluation shows that the proposed DroneNet shows superior performance on an equivalent CNN-based model.

==> figures/multifig.tex <==


%% Sample using subcaption
% \begin{figure}
% \centering
% \subfloat[\scriptsize Background noise (amplitude and spectrogram).]{\includegraphics[width=0.95\columnwidth]{figures/bg1_audio.pdf}} \\
% \subfloat[\scriptsize Bebop drone's signature (amplitude and spectrogram).]{\includegraphics[width=0.95\columnwidth]{figures/bebop_audio.pdf}}
% \caption{Sample acoustic signatures of background noise and two commercially available drone models (i.e., Bebop, Membo by Parrot) extracted from dataset \cite{sara2019}.}
% \label{fig:acoustic_signatures}
% \end{figure}
